Reconstructing higher-order interactions in coupled dynamical systems

Higher-order interactions play a key role for the stability and function of a complex system. However, how to identify them is still an open problem. Here, we propose a method to fully reconstruct the structural connectivity of a system of coupled dynamical units, identifying both pairwise and higher-order interactions from the system time evolution. Our method works for any dynamics, and allows the reconstruction of both hypergraphs and simplicial complexes, either undirected or directed, unweighted or weighted. With two concrete applications, we show how the method can help understanding the ecosystemic complexity of bacterial systems, or the microscopic mechanisms of interaction underlying coupled chaotic oscillators.

==> topletterhead11.tex <==
\vspace*{-1in}
\hspace*{-0.59in}\resizebox{3in}{!}{\includegraphics{qmlogo.eps}}\par

\vspace*{-0.9in}
\hspace*{4.9in}
\begin{minipage}[t]{1.95in}
\color{qmblue}
\raggedright
{\fontfamily{cmss}\fontsize{8}{9.25}\selectfont
\begin{tabbing}
T: \= +44 (0)20 7882 5440\kill
\textbf{School of Mathematical Sciences}\\
\textbf{Queen Mary, University of London}\\
Mile End Road, London E1 4NS\\
T: \= +44 (0)20 7882 5440\\
F: \> +44 (0)20 7882 7684\\
www.maths.qmul.ac.uk\\
\end{tabbing}
\vspace{-1ex}
%\textbf{School of Mathematical Sciences}\\
%\textbf{Professor Boris Khoruzhenko}\\
%Head of School\\
}
\end{minipage}
\color{black}

